A first engineering principles model for dynamical simulation of cement pyro-process cyclones

We provide a cyclone model for dynamical simulations in the pyro-process of cement production. The model is given as an index-1 differential-algebraic equation (DAE) model based on first engineering principle. Using a systematic approach, the model integrates cyclone geometry, thermo-physical aspects, stoichiometry and kinetics, mass and energy balances, and algebraic equations for volume and internal energy. The paper provides simulation results that fit expected dynamics. The cyclone model is part of an overall model for dynamical simulations of the pyro-process in a cement plant. This model can be used in the design of control and optimization systems to improve energy efficiency and reduce CO2 emission.

==> Nomenclature.tex <==

\printnomenclature

% Notation
\nomenclature{\(Q\)}{heat flow, $J/s$}
\nomenclature[N]{\(H\)}{enthalpy, $J$}
\nomenclature[N]{\(U\)}{internal energy, $J$}
\nomenclature[N]{\(P\)}{pressure, $bar$}
\nomenclature[N]{\(T\)}{temperature, $K$}
\nomenclature[N]{\(C\)}{concentration, $\frac{mol}{m^3}$}
\nomenclature{\(N\)}{material flux, $\frac{mol}{m^2s}$}
\nomenclature[N]{\(V\)}{volume, $m^3$}
\nomenclature{\(v\)}{velocity, $m/s$}
\nomenclature{\(J\)}{Diffusion, $\frac{mol}{m^2s}$}


\nomenclature{\(\hat{X}\)}{density of X, $\frac{[X]}{m^3}$}
\nomenclature{\(\tilde{X}\)}{flux of X, $\frac{[X]}{m^2s}$}
\nomenclature{\(\omega\)}{ rotational velocity, $\frac{r}{s}$}
\nomenclature{\(D_H\)}{ hydraulic diameter, $m$}
\nomenclature{\(D_e\)}{ effective diameter, $m$}

\nomenclature{\(n\)}{ amount of substance, $mol$}

\nomenclature{\(Re\)}{Reynold's number}
\nomenclature{\(E_A\)}{Activation energy, $J/mol$}
\nomenclature{\(x\)}{mole fraction}

\nomenclature{\(S\)}{stoichiometric coefficient matrix}
\nomenclature{\(r\)}{ reaction rate, $\frac{mol}{m^3s}$}
\nomenclature{\(R\)}{ production rate, $\frac{mol}{m^3s}$}
\nomenclature{\(m\)}{ mass, $kg$}
\nomenclature{\(\dot{m}\)}{mass rate, $kg/s$}

% physics
\nomenclature[P]{\( [x]\)}{unit of x}
\nomenclature[P]{\(\sigma\)}{Stefan-Boltzmann's constant, $5.670374419...*10^{-8}Wm^{-2}K^{-4}$}
\nomenclature[P]{\(\mu\)}{viscosity}
\nomenclature[P]{\(\rho\)}{mass density, $\frac{kg}{m^3}$}
\nomenclature[P]{\(M\)}{Molar weight, $\frac{g}{mol}$}
\nomenclature[P]{\(k\)}{conductivity, $\frac{J}{m s K}$}
\nomenclature[P]{\(c_m\)}{ molar thermal capacity}
\nomenclature[P]{\(\epsilon\)}{emissitivity}
\nomenclature[P]{\(\alpha\)}{absorptivity}
\nomenclature[P]{\(\alpha_B\)}{thermal diffusitivity}
\nomenclature[P]{\( V_{\sum} \)}{summed diffusion volume, $m^3$}

% Math
\nomenclature[M]{\(\Delta x\)}{difference of x, $[x]$}
\nomenclature[M]{\(\partial_x\)}{derivative w.r.t. x, $\pdv{}{x}$}

%Geometry
\nomenclature[G]{\(\theta\)}{ fill angle, $rad$}
\nomenclature[G]{\(\phi\)}{slope of bed height w.r.t. kiln axis, $rad$}
\nomenclature[G]{\(\psi\)}{kiln inclination angle}
\nomenclature[G]{\(\xi\)}{angle of bed repose}
\nomenclature[G]{\(A\)}{Area, $m^2$}
\nomenclature[G]{\(h\)}{ bed height,$m$}
\nomenclature[G]{\(V_{\Delta}\)}{ total segment volume,$m^3$}
\nomenclature[G]{\(r_c\)}{ kiln inner cross radius, $m$}
\nomenclature[G]{\(L\)}{ kiln length, $m$}
\nomenclature[G]{\(L_c\)}{ bed surface width, $m$}

 %subscripts / superscript
\nomenclature[S]{\(s\)}{Solid}
\nomenclature[S]{\(g\)}{Gas}
\nomenclature[S]{\(w\)}{Wall}
\nomenclature[S]{\(k\)}{Spatial location}
\nomenclature[S]{\(f\)}{fuel}
\nomenclature[S]{\(air\)}{air intake}
\nomenclature[S]{\(rad\)}{radiation}
\nomenclature[S]{\(cv\)}{convection}


